DISCERN: Decoding Systematic Errors in Natural Language for Text Classifiers

Despite their high predictive accuracies, current machine learning systems often exhibit systematic biases stemming from annotation artifacts or insufficient support for certain classes in the dataset. Recent work proposes automatic methods for identifying and explaining systematic biases using keywords. We introduce DISCERN, a framework for interpreting systematic biases in text classifiers using language explanations. DISCERN iteratively generates precise natural language descriptions of systematic errors by employing an interactive loop between two large language models. Finally, we use the descriptions to improve classifiers by augmenting classifier training sets with synthetically generated instances or annotated examples via active learning. On three text-classification datasets, we demonstrate that language explanations from our framework induce consistent performance improvements that go beyond what is achievable with exemplars of systematic bias. Finally, in human evaluations, we show that users can interpret systematic biases more effectively (by over 25% relative) and efficiently when described through language explanations as opposed to cluster exemplars.

==> contents/results/fully_trained.tex <==
\begin{table*}[]
    \parbox{0.6\linewidth}{
    \scalebox{0.7}{
    \centering
    \begin{tabular}{l|ccccc}
    \toprule
    \textbf{Dataset} & \multicolumn{5}{c}{\textbf{TREC}} \\
    \textbf{\# Aug. Ex.} &       \textbf{100} &      \textbf{200} &      \textbf{500} &     \textbf{1000} &     \textbf{2000} \\
    \midrule
    \textbf{No Exp.           } &   $\mathbf{89.18_{(1.36)}}$ &  $\mathbf{89.18_{(0.94)}}$ &  $89.09_{(1.88)}$ &  $89.09_{(1.88)}$ &  $89.09_{(1.88)}$ \\
    \textbf{SEAL*             } &   $88.91_{(1.11)}$ &  $88.91_{(1.27)}$ &  $\mathbf{89.18_{(1.24)}}$ &  $\mathbf{89.18_{(1.24)}}$ &  $\mathbf{89.18_{(1.24)}}$ \\
    \textbf{\textsc{{DiScErN}}} &   $89.00_{(1.28)}$ &  $89.18_{(0.77)}$ &  $89.09_{(0.63)}$ &  $89.09_{(0.63)}$ &  $89.09_{(0.63)}$ \\
    \bottomrule
    \end{tabular}
    }
    \caption{Accuracy of \texttt{distilbert-base-uncased} classifier after augmenting the training set with examples that have been generated using different approaches.}
    \label{tab:fully_trained_accuracy}
    }
    \quad
    \parbox{0.35\linewidth}{
    \scalebox{0.7}{
    \centering
    \begin{tabular}{l|ccc}
    \toprule
    \textbf{Dataset} & \multicolumn{3}{c}{\textbf{TREC}} \\
    \textbf{\# Aug. Ex.} &         \textbf{100} & \textbf{200} & \textbf{500}\\
    \midrule
    \textbf{Initial           } &     
    \multicolumn{3}{c}{27.27} \\
    \midrule
    \textbf{No Exp.           } &                \textbf{21.54} &        18.46 &        13.33 \\
    \textbf{SEAL*             } &                25.45 &        12.73 &        15.38 \\
    \textbf{\textsc{{DiScErN}}} &                23.08 &         \textbf{9.09} &        \textbf{10.91} \\
    \bottomrule
    \end{tabular}
    }
    \caption{\small Median misclassification rates of highly-erroneous clusters in fully trained classifiers post-training with examples obtained via data augmentation.}
    \label{tab:fully_trained_misclassification}
    }
\end{table*}


==> tables/distilbert_main.tex <==
\begin{table*}
    \centering
    \scalebox{0.95}{
    \begin{tabular}{l|cc|cc|cc}
    \toprule
    \textbf{Dataset $\rightarrow$} & \multicolumn{2}{c|}{\textbf{TREC (2000)}} & \multicolumn{2}{c|}{\textbf{AG News (1500)}} & \multicolumn{2}{c}{\textbf{Covid (4000)}} \\
    \textbf{\# Aug. Ex.} &      \textbf{500} &     \textbf{1000} &      \textbf{500} &     \textbf{1000} &      \textbf{500} &     \textbf{1000} \\
    \midrule
    Base & \multicolumn{2}{c|}{$58.48$} & \multicolumn{2}{c|}{$75.8$} & \multicolumn{2}{c}{$47.68$} \\
    \midrule
    % \textbf{Beam Explanations } &   $76.63_{(2.99)}$ &  $79.38_{(1.63)}$ &      $77.84_{(3.13)}$ &  $86.01_{(0.48)}$ &    $51.17_{(0.80)}$ &  $50.36_{(0.92)}$ \\
    No Desc. &  $77.09_{(2.18)}$ &  $78.04_{(1.74)}$ &  $80.03_{(1.51)}$ &  $80.68_{(1.08)}$ &  $51.07_{(0.66)}$ &  $48.08_{(1.14)}$ \\
    \discernf &  $76.99_{(2.49)}$ &  $78.98_{(1.88)}$ &  $79.75_{(1.25)}$ &  $80.96_{(1.98)}$ &  $51.12_{(0.64)}$ &  $48.60_{(1.36)}$ \\
    \discern &  $\mathbf{77.20_{(1.80)}}$ &  $\mathbf{79.21_{(1.53)}}$ &  $\mathbf{80.39_{(1.35)}}$ &  $\mathbf{83.44_{(1.00)}^\dagger}$ &  $\mathbf{51.55_{(0.47)}}$ &  $\mathbf{49.06_{(0.79)}}$ \\
    \bottomrule
    \end{tabular}
    }
    \caption{Accuracy of \texttt{distilbert-base-uncased} classifier after augmenting the training set with examples that have been generated using different approaches. Numbers in brackets next to dataset names indicate the number of training examples used for learning the initial classifier. \textbf{Bold} numbers indicate the best average classifier accuracy across five runs. $^\dagger$ indicates statistically significant improvement over other approaches using t-test. 
    % \ssr{At what p value limit?}. \rrm{standard 0.05 p-value. I think based off the social acceptance work, this is the accepted norm.}
    }
    \label{tab:dataset_generation}
\end{table*}
